Intriguing Properties of Modern GANs

Modern GANs achieve remarkable performance in terms of generating realistic and diverse samples. This has led many to believe that ``GANs capture the training data manifold''. In this work we show that this interpretation is wrong. We empirically show that the manifold learned by modern GANs does not fit the training distribution: specifically the manifold does not pass through the training examples and passes closer to out-of-distribution images than to in-distribution images. We also investigate the distribution over images implied by the prior over the latent codes and study whether modern GANs learn a density that approximates the training distribution. Surprisingly, we find that the learned density is very far from the data distribution and that GANs tend to assign higher density to out-of-distribution images. Finally, we demonstrate that the set of images used to train modern GANs are often not part of the typical set described by the GANs' distribution.

==> figures/LL-hists.tex <==
\begin{figure}
\begin{center}
    \includegraphics[width=\linewidth]{figures/LL_hists.pdf}
\end{center}
  \caption{Histograms of log-likelihood different GANs assign to different image groups.}
  \label{fig:LL-hists}

\end{figure}

==> figures/manifold-inference.tex <==
\begin{figure}
\begin{center}
    \includegraphics[width=.7\linewidth]{figures/manifold_inference.png}
\end{center}
  \caption{If GANs capture the true data manifold, it should be possible to use them for classification (left) and outlier detection (right). In both cases a sample $x$ is projected to the manifold, giving $\hat{x}_\theta$, and the distance between the original and the projection is used to infer the class or whether the sample is an outlier.}
  \label{fig:manifold-inference}

\end{figure}

==> supp_figures/OD_IN_AFHQ.tex <==
\begin{figure}
\begin{center}
    \includegraphics[width=.8\textwidth]{supp_figures/OD_IN_AFHQ.pdf}
\end{center}
  \caption{The GANs' performance on OD in ImageNet10, AFHQCat and AFHQDog, compared to the performance of the baselines.}
  \label{fig:app-OD-AFHQ}

\end{figure}

==> supp_figures/avg_OD.tex <==
\begin{figure}
\begin{center}
    \includegraphics[width=.8\textwidth]{supp_figures/avg_OD_fig.pdf}
\end{center}
  \caption{OD results when averaging over all labels. Here, again, the baseline models outperform the GANs investigated.}
  \label{fig:app-avg-OD}

\end{figure}

==> supp_figures/other_norms.tex <==
\begin{figure}
\begin{center}
    \includegraphics[width=.8\textwidth]{supp_figures/other_norms.pdf}
\end{center}
  \caption{Classification (top) and OD (bottom) performance for various different distance functions. The GANs perform poorly with all distance functions explored.}
  \label{fig:app-other-norms}

\end{figure}
